Maximum a posteriori signal recovery for optical coherence tomography angiography image generation and denoising

Optical coherence tomography angiography (OCTA) is a novel and clinically promising imaging modality to image retinal and sub-retinal vasculature. Based on repeated optical coherence tomography (OCT) scans, intensity changes are observed over time and used to compute OCTA image data. OCTA data are prone to noise and artifacts caused by variations in flow speed and patient movement. We propose a novel iterative maximum a posteriori signal recovery algorithm in order to generate OCTA volumes with reduced noise and increased image quality. This algorithm is based on previous work on probabilistic OCTA signal models and maximum likelihood estimates. Reconstruction results using total variation minimization and wavelet shrinkage for regularization were compared against an OCTA ground truth volume, merged from six co-registered single OCTA volumes. The results show a significant improvement in peak signal-to-noise ratio and structural similarity. The presented algorithm brings together OCTA image generation and Bayesian statistics and can be developed into new OCTA image generation and denoising algorithms.

==> responses <==
% Responses to reviewer comments

\begin{rebuttal}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% response to first reviewer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{response}{Response to the comments of Reviewer 1}
  \rcomment{C1}{Based on my understanding, the authors first proposed a probabilistic model (maximum likelihood estimation) to interpret and rationalize the empirical OCTA reconstruction techniques including AD and SV. Since it is difficult to directly incorporate prior knowledge in the conventional AD-OCTA or SV-OCTA, a maximum a posteriori estimate is thus used on the basis of the aforementioned MLE and regularization terms are proposed to improve the image quality. Whether or not this is what the authors would like to express, I would suggest the authors to reorganize and revise the methods section to better convey their ideas.
}{
  \begin{quote}
    We appreciate the reviewer's comment and acknowledge that the description was not sufficiently clear and confusing. In order to provide a clearer description to the reader, we reworked
    \begin{itemize}
        \item the introduction at \link{M1.1}, \link{M1.2}, and \link{M1.3},
        \item the method section at \link{M1.4}, and \link{M1.5},
        \item and also reinforced the point in the conclusion at \link{M1.8}, \link{M1.9}, and \link{M1.10}.
        \item We also moved the description of the regularizers from the algorithm section \link{M1.7} to the signal model section \link{M1.6}, to aid the reader's understanding.
    \end{itemize}
    To paraphrase: we extended an existing MLE for OCTA formulas to a MAP estimate for OCTA by including prior knowledge in the form of regularizers for denoising and improving image quality.
  \end{quote}
}
  \rcomment{C2}{
In section 1 and section 2.1, the authors have mentioned compressed sensing in multiple places. While I do understand that the MAP estimate used by the authors is somewhat equivalent to the CS in terms of denoising and the problem formulation. But I failed to see the immediate connection between CS and the main topic, since CS was not used to generate the results. I would suggest the authors to place those part in the appendix or supplementary materials.
  }{
  \begin{quote}
    The reviewer makes a valid point. Aspects of the reconstruction (inverse problem, regularizers that enforce sparsity) are related to compressed sensing but are not necessary or strictly relevant for the presented reconstruction algorithm. We removed references to compressed sensing in the following locations: 
    \begin{itemize}
        \item the abstract \link{M2.1},
        \item the method section \link{M2.2}, \link{M2.3}, \link{M2.4}, \link{M2.5}, \link{M2.6}, \link{M2.7}, and \link{M2.9},
        \item and the discussion section \link{M2.10}.
    \end{itemize}
    We added a paragraph, relating the reconstruction algorithm to compressed sensing, to the supplementary and refer to it in the method section at \link{2.8}.
  \end{quote}
  }
  \rcomment{C3}{
There are also some minor corrections need to be made
\begin{enumerate}
    \item[a.] In the second paragraph of section 3.2, multiple "\textmu{}" are not correctly displayed
    \item[b.] In the central column of Fig. 1., there should be 3 X fast scans and 3 Y fast scans, but now is 4 vs 2.
    \item[b.] In paragraph 4 of section 5, should be Fig. 1 instead of Fig. 14
\end{enumerate}
  }{
  \begin{quote}
    We appreciate the reviewer's attention to detail and corrected and our responses to the individual points are below:
    \begin{enumerate}
    \item[a.] There are three occurrences of the letter \textmu{} in section 3.2. We used the unicode character for \textmu{} in the latex file directly which may cause issues if the wrong character encoding is used. We replaced \textmu{} in all instances with the latex macro "\textbackslash textmu".
    \item[b.] The second scan from the top, right below the blue test scan, now represents an X-fast volume. X and Y-fast scans are now balanced, with three of each present. See the location \link{M3.5}.
    \item[b.] The reference is supposed to be "Fig. 3" and we corrected it accordingly. We assume "Fig. 1" may have been a typo by the reviewer. See \link{M3.10}
\end{enumerate}
    In addition to making the changes indicated by the reviewer above, we also updated the use of abbreviations for
    \begin{itemize}
        \item maximum likelihood estimate (MLE) at \link{M3.1}, \link{M3.2}, \link{M3.3}, and \link{M3.4},
        \item wavelet shrinkage (WS) at \link{M3.6} and \link{M3.8},
        \item total variation (TV) at \link{M3.7} and \link{M3.9}.
    \end{itemize}
  \end{quote}
}

\end{response}
\end{rebuttal}

